NaturalProver: Grounded Mathematical Proof Generation with Language Models

Theorem proving in natural mathematical language - the mixture of symbolic and natural language used by humans - plays a central role in mathematical advances and education, and tests aspects of reasoning that are core to intelligence. Yet it has remained underexplored with modern generative models. We study large-scale language models on two new generation tasks: suggesting the next step in a mathematical proof, and full proof generation. We develop NaturalProver, a language model that generates proofs by conditioning on background references (e.g. theorems and definitions that are either retrieved or human-provided), and optionally enforces their presence with constrained decoding. On theorems from the NaturalProofs benchmark, NaturalProver improves the quality of next-step suggestions and generated proofs over fine-tuned GPT-3, according to human evaluations from university-level mathematics students. NaturalProver is capable of proving some theorems that require short (2-6 step) proofs, and providing next-step suggestions that are rated as correct and useful over 40% of the time, which is to our knowledge the first demonstration of these capabilities using neural language models.

==> sections/related.tex <==
\section{Related Work}
Language models have been used for interactive theorem proving in formalized mathematics, in which proofs steps are verifiable and written in a programming language \citep{polu2020generative, polu2022formal,han2021proof,urban2020first}.
%
Previous work on informal theorem proving focuses on premise retrieval
\citep{ferreira2020natural,ferreira2020premise,welleck2021naturalproofs,han2021contrastive}, or informal-to-formal translation \citep{wang2020exploration}, which differs from generating next-steps or full proofs.
%
Outside of theorem proving, language models are used for problem solving \citep{saxton2018analysing,hendrycks2021measuring,cobbe2021gsm8k,wei2022chain},  math-related program synthesis  \citep{lample2020deep,austin2021program, drori2022neural} and competitive programming \citep{li2022competition}.
These settings generate executable programs or a numerical answer, which differ from our theorem proving setting, where the goal is generating arguments on many topics in natural mathematical language.
See \autoref{apx:related} for more related work.
%
